Finding Fair and Efficient Allocations When Valuations Don't Add Up

In this paper, we present new results on the fair and efficient allocation of indivisible goods to agents whose preferences correspond to {\em matroid rank functions}. This is a versatile valuation class with several desirable properties (such as monotonicity and submodularity), which naturally lends itself to a number of real-world domains. We use these properties to our advantage; first, we show that when agent valuations are matroid rank functions, a socially optimal (i.e. utilitarian social welfare-maximizing) allocation that achieves envy-freeness up to one item (EF1) exists and is computationally tractable. We also prove that the Nash welfare-maximizing and the leximin allocations both exhibit this fairness/efficiency combination, by showing that they can be achieved by minimizing any symmetric strictly convex function over utilitarian optimal outcomes. To the best of our knowledge, this is the first valuation function class not subsumed by additive valuations for which it has been established that an allocation maximizing Nash welfare is EF1. Moreover, for a subclass of these valuation functions based on maximum (unweighted) bipartite matching, we show that a leximin allocation can be computed in polynomial time. Additionally, we explore possible extensions of our results to fairness criteria other than EF1 as well as to generalizations of the above valuation classes.

==> sec5_ArbitAssign_Expts_old.tex <==
In this section, we introduce an extension of the envy-induced transfers (Algorithm~\ref{alg_bin}) to general valuations, as described in Algorithm \ref{alg_gen}.
Recall that the general principle is to iteratively eliminate envy by transfering an item from the envied bundle to the envied bundle until no agent is envied up to more than one item. 
Here at each iteration step, we transfer the item that induces the maximal increase in overall utility (see lines 3-6).
Note that, since agent $j$ loses one of her items, she may develop a positive marginal utility for a currently withheld item; in that case, the item in $A_0$ for which she has maximal marginal utility is given to her (see lines 6-8).
Note also that, for arbitrary utilities, if an agent $i$ acquires a new item $o$ due to an envy-induced transfer, at most one of her previous items, say $o^*$, may become unused, e.g. if $i$'s positive marginal utility for $o$ with her previous bundle $A_i$ was due to the fact that the individual who was assigned item $o^*$ has a higher utility for $o$ than $o^*$ and no other indivual prefers $o^*$ to its assigned item. In that case, item $o^*$ is revoked from agent $i$ and allocated to the agent with maximal and strictly positive marginal utility for it (see lines 10-13). If this creates another unused item, we repeat the process until there are no unused items or the unused item has zero marginal utility for all agents -- in the latter case, the unused item is added to the withheld set (see lines 14-18).

We now provide numerical results to compare the loss incurred by Algorithm~\ref{alg_gen} and that of $P_L$ the extension of \cite{lipton2004approximately} algorithm to groups of agents, as presented in \cite{benabbou2019fairness}. The performances of these procedure are estimated both in terms of percentage of items wasted (Waste) and price of fairness (PoF) which is formally defined as follows:
$$PoF(P) = \frac{\max \{\USW(A) \ | \ A \mbox{ is an allocation}\}}{\USW(A(P))}$$
where $A(P)$ is the allocation returned by a given procedure $P$. 
In our experiments, we use the dataset called ``MovieLens-ml-1m'' which contains approximately 1,000,000 ratings (from $0$ to $5$) of 4,000 movies made by 6,000 users \cite{movieLens}. To generate an instance of our allocation problem, we select $200$ movies at random ($|O|=200$)  and then we only consider the users that rated at least one of these movies. We use the user ratings as individual utilities.
We consider the following user partitions:
\begin{itemize}
	\item Gender: 2 agents (male or female),
	\item Age: $7$ agents representing the $7$ age-groups,
\end{itemize}
and the following agents' valuations:
\begin{itemize}
	\item Ratings: $$v_i(S) = \max \{\, \sum\limits_{u \in N_i} r_{u,\pi(u)} \mid \pi \in \Pi(N_i,S) \,\}$$ where $r_{uo}$ is the rating of movie $o$ made by user $u$,
	\item Norm: $v'_i(S)= v_i(S)/v_i(O)$,
\end{itemize}
for all agents $i \in N$ representing a group of users and for all bundles of movies $S \subseteq O$. The results given in Table \ref{tabTests} are averaged over 50 runs.

In Table \ref{tabTests}, we observe that $P_L$ the extension of \cite{lipton2004approximately} algorithm to groups may be wasteful but in practice it has almost zero-waste and also good PoF (the lower the better). In comparison, Algorithm~\ref{alg_gen} the extension of the envy-induced transfers to general valuations is guaranteed to be non-wasteful but in practice it has larger PoF than $P_L$. 



\begin{algorithm} \small
	\DontPrintSemicolon
	\caption{\small Envy-Induced Transfers for general valuations\label{alg_gen}}
	Compute a clean, socially optimal allocation.\\						
	\textbf{/**Envy-Induced Transfers and Reallocations**/}\\
	\While{$\exists i,j \in N$ such that $i$ envies $j$ up to more than $1$ item}
	{
		Pick $i$, $j$, $o$ maximizing $\Delta_i(A_i;o) + \Delta(A_j;o)$ over all $i,j \in N$ and all $o \in O$ such that $i$ envies $j$ more than $1$ item and $\Delta_i(A_i;o)>0$.\\ 		
		$A_j \leftarrow A_j \backslash \{o\}$; $A_i \leftarrow A_i \cup \{o\}$.\\
		\If{$\exists o \in A_0$ such that $\Delta_j(A_j;o)>0$}
		{Pick $o \in A_0$ that maximizes $\Delta_j(A_j;o)$.\\ $A_j \leftarrow A_j \cup \{o\}$.}
		\If{$\exists o^* \in A_i$ that is unused}
		{$A_i \leftarrow A_i \backslash \{o^*\}$; revoked = \textbf{true}.\\
		\While{revoked \!\! = \!\! \textbf{true} \textbf{and} $\exists k$ s.t. $\Delta(A_k;o^*)\! >\! 0$}{
			Allocate $o^*$ to agent $k$ maximizing $\Delta(A_k;o^*)$.\\
			\lIf{$\exists o \in A_k$ that is unused}{\\
				\hspace{0.5cm}$A_k \leftarrow A_k \backslash \{o\}$; $o^* \leftarrow o$.
			} 
			\lElse{revoked = \textbf{false}.}
		}
		\lIf{revoked = \textbf{true}}{$A_0 \leftarrow A_0 \cup \{o^*\}$.}
        }
    }
%	}			
\end{algorithm}





\begin{table}[h]
\centering
\begin{tabular}{ c | c| c c | c c }
 & & \multicolumn{2}{c|}{$P_L$} &   \multicolumn{2}{c}{Algorithm~\ref{alg_gen}}  \\
 &  Types &  Ratings  & Norm  & Ratings  & Norm  \\ \hline
 PoF & Age &  1.01 & 1.15  & 1.05 & 1.19 \\ 
 Waste& Age &  1.25 & 0.20 & 0.00 & 0.00  \\ \hline
  PoF  & Gender &  1.00 & 1.02  & 1.00 & 1.03 \\ 
 Waste  & Gender & 0.00 & 0.00 & 0.00 & 0.00 \\
\end{tabular} 
\caption{Performances of allocation procedures. \label{tabTests}}
\end{table}



